Rule-based Graph Repair using Minimally Restricted Consistency-Improving Transformations

Model-driven software engineering is a suitable method for dealing with the ever-increasing complexity of software development processes. Graphs and graph transformations have proven useful for representing such models and changes to them. These models must satisfy certain sets of constraints. An example are the multiplicities of a class structure. During the development process, a change to a model may result in an inconsistent model that must at some point be repaired. This problem is called model repair. In particular, we will consider rule-based graph repair which is defined as follows: Given a graph $G$, a constraint $c$ such that $G$ does not satisfy $c$, and a set of rules $R$, use the rules of $\mathcal{R}$ to transform $G$ into a graph that satisfies $c$. Known notions of consistency have either viewed consistency as a binary property, either a graph is consistent w.r.t. a constraint $c$ or not, or only viewed the number of violations of the first graph of a constraint. In this thesis, we introduce new notions of consistency, which we call consistency-maintaining and consistency-increasing transformations and rules, respectively. This is based on the possibility that a constraint can be satisfied up to a certain nesting level. We present constructions for direct consistency-maintaining or direct consistency-increasing application conditions, respectively. Finally, we present an rule-based graph repair approach that is able to repair so-called \emph{circular conflict-free constraints}, and so-called circular conflict-free sets of constraints. Intuitively, a set of constraint $C$ is circular conflict free, if there is an ordering $c_1, \ldots, c_n$ of all constraints of $C$ such that there is no $j <i$ such that a repair of $c_i$ at all graphs satisfying $c_j$ leads to a graph not satisfying $c_j$.

==> Algorithms/algo_randomized.tex <==
\begin{figure}
\centering
\begin{algorithm}[H]
	%\DontPrintSemicolon
	\KwData{A graph $G$, a conflict free constraint in UANF and a repairing set $\mathcal{R}$ for each layer $\kmax  < k \nlvl(c)$}
	\KwResult{A graph $H$ with $H \models c$}
	$\mathcal{G} \gets \{G\}$	
	\For{$i = 0$ \KwTo $m$}{
		\ForEach{$G\in \mathcal{G}$}{
			\ForEach{$t: G \Longrightarrow H$}{
				\If{$H \models c$}{
					\KwRet{H}
				}
				\If{$t$ is non-consistency decreasing 
					or consistency increasing}{
					
					$\mathcal{G} \gets \mathcal{G} \cup \{H\}$\; 			
				
				}
			}
		}
					
		}
	


\caption{Repair for conflict free constraints and repairing set}\label{Algo_randomized}

\end{algorithm}
\end{figure}

==> Kapitel/RuleSets/generation_repairing_rule_set.tex <==
\subsection{Construction of Repairing Sets}

In the following we want to introduce a construction of these 
repairing sets for a given circular conflict free constraint in UANF. 

\begin{definition}[\textbf{constructed repairing set}]\label{def_constr_rep}
	Let a circular conflict free constraint $c$ in UANF with $\nlvl(c) > 1$ or 
	$c = \forall(C_1, \false$ and $E_{C_1} \neq \emptyset$ be given. 
	The \emph{constructed repairing set}, $\mathcal{R}$, for $c$ is constructed 
	in the following way.
	For each universally bound graph $C_k$ of $c$  and every pair of graphs 
	$C, C' \ig{C_{k-1}}{C_k}$ with $C$ being a sub-graph of $C'$ there does 
	exist a rule 
	$$ \rle{C'}{a_{k-1}^r}{C}{\id}{C}$$
	in $\mathcal{R}$. 
	For each existentially bound graph $C_k$ of $c$ and every pair of graphs
	$C, C' \in \ig{C_{k-1}}{C_k}$ with $C$ being a sub-graph of $C'$ there does 
	exist a rule  
	$$\rle{C}{\id}{C}{a_{k-1}^r}{C'}$$ 
	in $\mathcal{R}$.
\end{definition}
Note that for each element of existentially bound graphs, $\mathcal{R}$ contains a rule that only inserts this element, and for each element of universally bound graphs $\mathcal{R}$ contains a rule that only removes this element. 

\begin{theorem}
	Let a circular conflict free constraint $c$ in UANF with $\nlvl(c) > 1$ 
	or $c = \forall(C_1, \false)$ and $E_{C_0} \neq \emptyset$ be given. 
	The set of rules constructed by Definition \ref{def_constr_rep} is a 
	repairing set w.r.t. $c$.
\end{theorem}
\begin{proof}
	Let $\mathcal{R}$ be the constructed rule set.
	If $\nlvl(c)= 1$ and $E_{C_1}\neq \emptyset$, there does exist a rule
	$\rho = \rle{C_1}{a_0^r}{C'}{\id}{C}$ with $C \in \ig{\emptyset}{C_1}$ 
	such that $V_C = V_{C_0}$. Then,
	$$C_1 \Longrightarrow_{\rho,\id} C$$ 
	is a repairing sequence for $C_1$ and $\mathcal{R}$ is a repairing rule set 
	for $c$. 
	
	If $	\nlvl(c) \geq 2$, consider an existentially bound graph $C_k$ 
	and the transformation sequence 
	$$C_{k-1} \Longrightarrow_{\rho_1, m} C_{k}$$
	with $\rho_1 = \rle{C_{k-1}}{\id}{C_{k-1}}{a_{k-1}}{C_k}$. 
	If $C_k$ has no conflict with an universally bound graph $C_j$ with 
	$j < k$, $C_k \models_k c$ and this is a repairing sequence. 
	If, $C_k \not \models_k c$, an occurrence $p$ of an universally bound graph 
	$C_j$ with $j < k$ has been inserted.
	Then, the repairing sequence can be extended by 
	$$C_k \Longrightarrow_{\rho_2,m} G_1$$ 
	with $\rho_2 = \rle{C}{\id}{C}{a_j^r}{C_{j+1}}$ such that $C \in \ig{C_j}
	{C_{j+1}}$ and $V_C = V_{C_{k+1}}$. with $p = m \circ a_{j-1}^r$.
	Since $j< k$, such a match and transformation must exist.
	If this inserts new occurrences of universally bound graphs $C_{j'}$ with 
	$j' < k$, we repeat this process.
	 
	
	 
\end{proof}


\begin{example}

\end{example}



==> Kapitel/basic_improving_rules/comparison_basic_rules.tex <==
\subsection{Comparison with other consistency concepts and basic increasing rules}

\input{figures/consistency_relations_basic_rules.tex}

Before we continue with the construction of application conditions for basic increasing rules, let us once more compare the notion of direct consistency increasing with the notions of (direct) consistency improving and sustaining and consistency guaranteeing and preserving with the restriction that only basic increasing rules are used. 
The results of these differ from the results of chapter \ref{comp_general} and are displayed in figure \ref{fig:consistency_relations_basic}.
It can be seen that in the case of basic increasing rules  the notions of direct consistency increasing and direct consistency improving are related in the sense that improving implies direct increasing and therefore direct increasing is a finer notion than improving. 

Additionally, with lemma \ref{lemma:equiv_direct_normal} follows immediately that guaranteeing implies direct increasing. 
We show that improving implies (direct) increasing and that (direct) increasing does not imply sustaining which also implies that increasing does not imply improving since each improving transformation is also a sustaining one. 
\begin{lemma}
Let a constraint $c$ in UANF, a basic increasing rule $\rho$ and a transformation $t: G \Longrightarrow_{\rho} H$ be given. 
Then, 
\begin{equation*}
	\begin{split}
		&t \text{ is improving w.r.t $c$ } \implies t \text{ is direct consistency increasing w.r.t $c$ } \wedge \\
		&t \text{ is direct increasing w.r.t $c$ } \centernot \implies t \text{ is consistency sustaining w.r.t $c$}
	\end{split}
\end{equation*}
\end{lemma}

\begin{proof}
\begin{enumerate}
\item Let $t$ be a consistency improving transformation w.r.t $c$. 

\end{enumerate}
\end{proof}

==> Kapitel/partial_improving/partial_improving_old.tex <==
\subsection{partial consistency improving}

\begin{definition}[\textbf{improving atomic transformation}]
Given a graph $G$ a condition $c$ over $C_0$ and a morphism $p: C_0 \to G$ with $p \not \models c$.
An \emph{atomic transformation} is a rule application that inserts or deletes one single element. 
A set of  atomic transformations is called \emph{improving set} if the morphism $p': C_0 \to H$ with $p = p'$ and $H$ being the graph derived by applications of all transformations in $A$ satisfies $c$. 
$A$ is called a \emph{minimal improving set} if no improving set $B \subset A$ exists. 
Let $I_{c,p}$ be the set of all minimal improving sets for $G$ with respect to $c$ and $p$. 
A set $A \in I_{G,c}$ with $|A| \leq |A'|$ for all $A' \in I_{c,p}$ is called a \emph{least changing minimal improving set}.
The total number of improving atomic transformations for $G$ and $p$ with respect to $c$ is given by $$\iat_p(G,c) :=  \sum_{A \in I_{G,c}} |A |$$
If $c$ is a constraint the following notation is used:
$$\iat(G,c) :=  \sum_{A \in I_{G,c}} |A |$$
\end{definition}

%\begin{definition}[\textbf{improving atomic transformation}]
%Given a graph $G$ and a constraint $c$. 
%An \emph{atomic transformation} is a rule application that inserts or deletes one single element. 
%A set of atomic transformations is called \emph{improving set} if the graph derived by application of all transformations in $A$ satisfies $c$,
%$A$ is called a \emph{minimal improving set} if no improving set $B \subset A$ exists. 
%Let $I_{G,c}$ be the set of all minimal improving sets for $G$ regarding $c$.
%A set $A \in I_{G,c}$ with $|A| \leq |A'|$ for all $A' \in I_{G,c}$ is called a \emph{least changing minimal improving set}.
%The total number of improving atomic transformations  for $G$ regarding $c$ is given by $$\iat(G,c) := | \bigcup_{A \in I_{G,c}} A |$$ 
%\end{definition}

\begin{definition}[\textbf{partial consistency improving transformation}]\label{def_partial_imp}
Given a constraint $c$ and a rule $r$, a transformation $G \xRightarrow{r,m} H$ is \emph{partial consistency improving} with repect to $c$ if $\iat(H,c) < \iat(G,c)$.  


\end{definition}


%\begin{construction}
%Let a graph $G$ and a condition $c$ in ANF be given. 
%We calculate $\iat(G,c)$ in the following way:
%\begin{enumerate}
%	\item $c = \true$, for $p: P \to G$:
%		$$\rep(c, p) := 0$$
%	\item $c = \false$, for $p : P \to G$:
%	$$\rep(c,p) := 0$$			
%	\item $c = \forall(a:C_0 \inj C_1, d)$, let $e :=  \exists(a:C_0 \inj C_2, \neg d)$:
%		\begin{enumerate}
%			\item For $p: C_0 \to G$:
%				%$$\rep(c,p) := |C_1| + \sum_{\substack{p = q \circ a \\ q \models \neg d}}\rep(d, q)$$
%				$$\rep(c,p) := \begin{cases}
%					0, p \models e \\
%					|C_1| + \sum_{\substack{p = q \circ a}}\rep(d, q)
%				\end{cases}$$
%			\item $$repair(c) := \sum_{\substack{p : C_0 \to G \\ p \models e}} \rep(c,p)$$
%		\end{enumerate}
%	\item $c = \exists(a:C_0 \inj C_1,d)$:
%		\begin{enumerate}
%			\item For $p: C' \to G$ with $C' \subseteq C_0$, $p \models \exists(a': C' \inj Q, \true) \leq \exists(a: C_0 \inj C_1, \true)$ and $d'$ being the closest partial morphism of $d$ over $Q$.
%				$$\rep(c,p) := |C_1| - |Q| + \sum_{\substack{p = q \circ a'}}\rep(d',q)$$
%				
%			\item $$\rep(c) := \sum_{\substack{p : C' \to G \\ C' \subseteq C_0}} \rep(c,p)$$ 
%		\end{enumerate}
%		
%	%\item $c = d_1 \wedge d_2$ or $c = d_1 \vee d_2$:
%	%		$$\rep(c) := \rep(d_1) + \rep(d_2)$$
%	
%\end{enumerate}
%\end{construction}

%\begin{construction}\label{const_rep}
%Let a graph $G$ and a condition $c$ in ANF be given. 
%\begin{enumerate}
%	\item $c = \true$ for $p: P \inj G$:
%		$$\rep_G(c,p) := 0$$
%	\item $c = \false$ for $p: P \inj G$:
%		$$\rep_G(c,p) := 0$$
%	\item $c = \forall(a:C_0 \inj C_1, d)$, let $e := \exists(a:C_0 \inj C_1, \neg d)$:
%	\begin{enumerate}
%		\item For $p: C_0 \inj G$:
%		$$\rep_G(c,p) := 	|E_{C_1}| + |\iso(C_1)| + \sum_{\substack{p = q \circ a \\ q \models \neg d}} \rep_G(d,q) $$
%		\item $$ \rep_G(c) := \sum_{\substack{p : C_0 \inj G \\ p  \models e}} \rep_G(c,p)$$
%	\end{enumerate}
%	
%	 \item $c = \exists(a: C_0 \inj C_1, d)$:
%	 \begin{enumerate}
%	 	\item For $p: C' \inj G$ with $C' \subseteq C_0$,$p \models \exists(a':C' \inj Q, \true) \leq \exists(a:C_0 \inj C_1, \true)$
%	 	$$\rep_G(c,p) := |C_1| - |Q| + \sum_{H \in \overlay_p(G, C_1)} \rep_H(d, q')$$
%	 	\item $c = \exists(a: \emptyset \inj C_1,d)$ 
%	 	$$\rep_G(c) := \sum_{\substack{p: C' \inj G \\ C' \subseteq C_1}} \rep_G(c,p) $$
%	 \end{enumerate}
%	
%\end{enumerate}
%
%\end{construction}

\begin{construction}\label{const_rep}
Let a graph $G$ and a condition $c$ in ANF be given.
\begin{enumerate}
	\item $c = \true$ and $p: C_0 \to G$:
		$$ \rep(c,p) := 0$$
	
	\item $c = \false$ and $p: C_0 \to G$:
		$$ \rep(c,p) := 0$$
	\item $c = \forall(a:C_0 \inj C_1, d)$ and $p: C_0 \to G$:
		\begin{enumerate}
			\item $p \models c$:
				$$\rep(c,p) = 0$$
			\item$p \not \models c$: 
			Let $Q$ be the set of morphisms $q: C_1 \to G$ with $p = q  \circ a$ and $q \not \models d$.
				$$\rep(c,p) := | \bigcup_{q \in Q} q(E_{C_1 \setminus C_0}) \cup q(\iso(C_1) \cap V_{C_1})| + \sum_{q \in Q} \rep(d,q)$$
		\end{enumerate}				
		
		
	\item $c = \exists(a: C_0 \inj C_1,d)$ and $p: C_0 \to G$:
		$$\rep(c,p) := \begin{cases}
						0 &, p \models c \\
						\sum_{\substack{q: C'_1 \to G \\ p = q \circ a \\ C'_1 \subseteq C_1}}\sum_{\substack{H \in \overlay_q(G,C_1)\\ q':C_1 \to H \\ q \leq q'}} |C_1| - |C'_1| + \rep(q',d) &, p \not \models c
		
						\end{cases}$$
\end{enumerate}
\end{construction}

\begin{lemma}
Let a graph $G$ and a condition $c$ over $C_1$ in ANF and a morphism $p: C_1 \to G$ be given. The value $\rep(c,p)$ of construction \ref{const_rep} is an upper bound for $\iat_p(G,c)$.
\end{lemma}
\begin{proof}
\begin{enumerate}
\item $c = \true$:
	The morphism $p$ satisfies $\true$ and therefore $\iat(p,c) = 0 = repair(c,p)$.
\item  $c = \false$:
	There is no set of improving transformations, such that $p \models c$ and therefore $\iat(p,c) = 0 = repair(c,p)$.

\item $c = \forall(a:C_0 \inj C_1, d)$:
	For every morphism $q:C_1 \to G$ with $q \not \models d$ and $p = q \circ a$ repair sets exists that either (a) delete nodes or edges of $C_1 \setminus C_0$ or (b) repair, such that $q \models d$. 
	\begin{enumerate}
		\item For every $q$ minimal improving sets exists that delete exactly one edge or isolated node of $G$. 
			  The sum of these minimal improving sets is therefore bound by $$\sum_{\substack{q: C_1 \to G \\ p = q \circ a \\ q \not \models d}} |C_1 \setminus C_0|$$.
		
		\item For every $q$ minimal improving sets exists that repair $d$. By the induction hypothesis the sum of these sets has the upper bound: $$\rep(d,q)$$ 
		With (a) and (b) $\iat(p,c) \leq \rep(c,p)$ follows. 
	\end{enumerate}
	
\item $c = \exists(a:C_0 \inj C_1, d)$:
	For every morphism $q: C'_1 \to G$ with $p = q \circ a$ and $C'_1 \subseteq C_1$ minimal improving sets exist that (a) insert the necessary elements of $C_1 \setminus C'_1$ and afterwards (b) repair, such that $q \models d$. 
	\begin{enumerate}
		\item For every $q$ every possible insertion of the elements of $C_1 \setminus C'_1$ is performed in one minimal improving set. Therefore the sum of these operations is exactly $$(|C_1| - |C'_1|)|\overlay_q(G, C_1)|$$
		\item After the insertions in (a) a minimal improving set exists that repairs $d$ for the morphism $q': C_1 \to H$ with $q \leq q'$ for every $H \in \overlay_q(G,C_1)$.
		Therefore, the sum of these sets has, by induction hypothesis, the upper bound $$\sum_{\substack{H \in \overlay_p(G,C_1) \\ q': C_1 \to G \\ q \leq q}} repair(q',d)$$
		With (a) and (b) follows: 
		\begin{align*}
			\iat(p,c) &\leq \sum_{\substack{q: C'_1 \to G \\ p = q \circ a \\ C'_1 \subseteq C_1}}(|C_1| - |C'_1|)|\overlay_q(G, C_1)| + \sum_{\substack{H \in \overlay_p(G,C_1) \\ q': C_1 \to G \\ q \leq q}} \rep(q',d)\\
			 &= \sum_{\substack{q: C'_1 \to G \\ p = q \circ a \\ C'_1 \subseteq C_1}}\sum_{\substack{H \in \overlay_q(G,C_1)\\ q':C_1 \to H \\ q \leq q'}} |C_1| - |C'_1| + \rep(q',d)\\
			 &= \rep(c,p)
		\end{align*}
	\end{enumerate}
\end{enumerate}
\end{proof}

\begin{lemma}
Given a constraint $c$, a rule $r$ and a graph $G$.
A transformation $G \xRightarrow{r,m} H$ is partial consistency improving if $\rep_G(c) < \rep_H(c)$.
\end{lemma}
\begin{proof}
Noch ein ganz super duper noicer proofböärt
\end{proof}

==> Kapitel/repair/non-repairing_set.tex <==
\subsection{Rule based repair for non-repairing sets}
\input{Algorithms/algo_randomized}

==> figures/fig_counterexamples_guaranteeing.tex <==
\begin{figure}
\includegraphics[scale=0.8]{figures/images/counterexample_direct_guaranteeing}
\caption{example}\label{fig:counterexamples_guaranteeing_maintaining}
\end{figure}
